FedGroup: Efficient Clustered Federated Learning via Decomposed Data-Driven Measure

Federated Learning (FL) enables the multiple participating devices to collaboratively contribute to a global neural network model while keeping the training data locally. Unlike the centralized training setting, the non-IID and imbalanced (statistical heterogeneity) training data of FL is distributed in the federated network, which will increase the divergences between the local models and global model, further degrading performance. In this paper, we propose a novel clustered federated learning (CFL) framework FedGroup, in which we 1) group the training of clients based on the similarities between the clients' optimization directions for high training performance; 2) construct a new data-driven distance measure to improve the efficiency of the client clustering procedure. 3) implement a newcomer device cold start mechanism based on the auxiliary global model for framework scalability and practicality. FedGroup can achieve improvements by dividing joint optimization into groups of sub-optimization and can be combined with FL optimizer FedProx. The convergence and complexity are analyzed to demonstrate the efficiency of our proposed framework. We also evaluate FedGroup and FedGrouProx (combined with FedProx) on several open datasets and made comparisons with related CFL frameworks. The results show that FedGroup can significantly improve absolute test accuracy by +14.1% on FEMNIST compared to FedAvg. +3.4% on Sentiment140 compared to FedProx, +6.9% on MNIST compared to FeSEM.

==> Convergence.tex <==
\section{Convergence Analysis}\label{sec:convergence}

We analyze convergence for FedGroup in this section. First, we analyze the convergence of our proposed framework without inter-group aggregation (e.g. $\eta_g=0$ in Algorithm~\ref{alg:fedgrouprox} line 10), and then extend it to the case with inter-group aggregation.

In FedGroup, the group membership for each group is static, so we can assume that any client $k$ is allocated to group $g$.
We make the following assumptions on the local loss function $F_{k,g}(\cdot)$ for any client $k$.


\begin{assumption}\label{assu1}
	For any client $k$, $F_{k,g}(\cdot)$ is convex.
\end{assumption}

\begin{assumption}\label{assu2}
	$F_{k,g}$ is $M$-Lipschitz continuous: for all $\bm{w}$ and $\bm{v}$, $\|F_{k,g}(\bm{w})-F_{k,g}(\bm{v})\| \leq M\|\bm{w}-\bm{v}\|$.
\end{assumption}

\begin{assumption}\label{assu3}
	$F_{k,g}$ is $L$-Lipschitz smooth: for all $\bm{w}$ and $\bm{v}$, $\|\nabla F_{k,g}(\bm{w})-\nabla F_{k,g}(\bm{v})\| \leq L\|\bm{w}-\bm{v}\|$.
\end{assumption}

The above assumptions have been made by many relevant works~\cite{lee2020tornadoaggregate, liu2020client, wang2019adaptive}.

\begin{definition}[Group Loss Function]\label{def1}
	For any group $g\in \mathcal{G}$, the group loss function is $F_g(\cdot) \triangleq \sum_{k}p_kF_{k,g}(\cdot)$, and $\sum_{k}p_k=1$.
\end{definition}

\begin{lemma}
	Under Assumptions~\ref{assu1} to \ref{assu3}, the group loss function $F_g$ are convex, $M$-Lipschitz continuous, $L$-Lipschitz smooth for any $g$.
\end{lemma}

\textit{Proof.} This simply follows by Definition~\ref{def1}, given $F_g(\cdot)$ is a linear combination of the local loss function $F_{f,g}(\cdot)$.


Let $w_t^g$ be the model parameter maintained in the group $g$ and at the $t$-th step. Let $e$ be the current local epoch number, $e \in [0, E]$.  We assume that the $0$-th local epoch is the synchronization step, so $e$ will be reset before the start of the communication round $t$. Then the update of FedGroup without inter-group aggregation can be described as:
	
\begin{equation}
\label{eq:fedgroup without agg}
\begin{aligned}
	\bm{w}_{t,e}^{k,g}&=
	\begin{cases}
		\bm{w}_t^g, & e=0\\
		\bm{w}_{t,e-1}^{k,g}-\eta\nabla F_{k,g}(\bm{w}_{t,e-1}^{k,g}), &e\in[1,E]
	\end{cases}\\
	\bm{w}_t^g &\triangleq \sum_{k}p_k\bm{w}_{t,E}^{k,g}
\end{aligned}
\end{equation}

Here we introduce an additional notation \textit{virtual group model} $\bm{v}_{t,e}^g$ to measure the divergence between federated training and SGD-based centralized training, which is motivated by~\cite{stich2018local, Li2020On, lee2020tornadoaggregate}. We assume that there is a virtual group model $\bm{v}_{t,e}^g$ that is centralized trained on the collection of members' data and is synchronized with the federated model in each communication round. We introduce this notion formally below.

\begin{equation}
	\bm{v}_{t,e}^{g}=
	\begin{cases}
		\bm{w}_t^g, & e=0\\
		\bm{v}_{t,e-1}^{g}-\eta\nabla F_{g}(\bm{v}_{t,e-1}^{g}), &e\in[1,E]
	\end{cases}
\end{equation}

\begin{definition}[Intra-Group Gradient Divergence]
\label{def2}
Given a certain group membership, for any $g$ and $k$, $\delta_{k,g}$ represents the gradient difference between the loss functions of client $k$ and group $p$, as expressed below:
	\begin{equation}
		\delta_{k,g} \triangleq \max_{\bm{w}}\|\nabla F_{k,g}(\bm{w})-\nabla F_g(\bm{w})\|
	\end{equation}
And the intra-group gradient divergence is defined as Eq.~(\ref{eq:intra-group gradient divergence}),
	\begin{equation}
		\label{eq:intra-group gradient divergence}
		\delta \triangleq \sum_{g\in \mathcal{G}}~\sum_{k\in g.clients} p_g p_k \delta_{k,g}
	\end{equation}
\end{definition}

\begin{lemma}[Upper bound of the divergence of $\bm{w}_{t,e}^{k,g}$]
	\label{lem2}
	Let Assumptions~\ref{assu1} to \ref{assu3} hold, the upper bound of divergence between the FedGroup model and the virtual group model for any $t$, $e$ is given by
\begin{equation}
	\|\bm{w}_{t,e}^{k,g}-\bm{v}_{t,e}^g\| \leq \frac{\delta_{k,g}}{L}((\eta L+1)^{e}-1)
\end{equation}
\end{lemma}

\textit{Proof.} By the smoothness of $F_{k,g}(\cdot)$ and the Definition~\ref{def2}, we have

\begin{equation}
	\label{eq:bouding proof}
	\begin{aligned}
		&\|\bm{w}_{t,e}^{k,g}-\bm{v}_{t,e}^g\| \\
		&= \|\bm{w}_{t,e-1}^{k,g}-\eta\nabla F_{k,g}(\bm{w}_{t,e-1}^{k,g})- \bm{v}_{t,e-1}^g + \eta\nabla F_{g}(\bm{v}_{t,e-1}^{g})\| \\
		&\leq\| \bm{w}_{t,e-1}^{k,g} - \bm{v}_{t,e-1}^g \| + \eta \| \nabla F_{k,g}(\bm{w}_{t,e-1}^{k,g}) - \nabla F_{g}(\bm{v}_{t,e-1}^{g}) \| \\
		&\leq\| \bm{w}_{t,e-1}^{k,g} - \bm{v}_{t,e-1}^g \| + \eta \| \nabla F_{k,g}(\bm{w}_{t,e-1}^{k,g}) - \nabla F_{k,g}(\bm{v}_{t,e-1}^{g}) \| \\
		&~~~ +\eta \| \nabla F_{k,g}(\bm{v}_{t,e-1}^{g}) - \nabla F_{g}(\bm{v}_{t,e-1}^{g}) \| \\
		&\leq (\eta L +1) \| \bm{w}_{t,e-1}^{k,g} - \bm{v}_{t,e-1}^g \| + \eta \delta_{k,g}
	\end{aligned}
\end{equation}

Let $h(e)= \|\bm{w}_{t,e}^{k,g}-\bm{v}_{t,e}^g\| $, then we can rewrite Eq.~(\ref{eq:bouding proof}) as
\begin{equation}
	\begin{aligned}
		&h(e) \leq (\eta L+1)h(e-1)+\eta\delta_{k,i} \\
		&\frac{h(e)+\delta_{k,g}/L}{h(e-1)+\delta_{k,g}/L} \leq \eta L +1
	\end{aligned}
\end{equation}

Given that $h(0) = \|\bm{w}_{t,0}^{k,g}-\bm{v}_{t,0}^g\| = 0$, by induction, we have
\begin{equation}
	g(e) + \frac{\delta_{k,g}}{L} \leq \frac{\delta_{k,g}}{L}(\eta L +1)^e
\end{equation}
Therefore, Lemma~\ref{lem2} is proved. \hfill$\square$

Combing Lemma~\ref{lem2} and Eq.~(\ref{eq:fedgroup without agg}) and using Jensen's inequality we get
\begin{equation}
	\label{eq:different between group and virtual}
	\begin{aligned}
	\| \bm{w}_t^g -\bm{v}_{t,e}^g \| &\leq \sum_{k} p_k \| \bm{w}_{t,E}^{k,g} - \bm{v}_{t,e}^g \| \\
	&\leq \frac{\delta}{L}((\eta L+1)^{E}-1)
	\end{aligned}
\end{equation}

Consider the continuous of $F_g(\cdot)$ we have

\begin{equation}
	\label{eq:bound fedgroup without agg}
	\| F_g(\bm{w}_t^g) - F_g(\bm{v}_{t,e}^g) \| \leq \frac{\delta M}{L}((\eta L+1)^{E}-1)
\end{equation}

\begin{theorem}[Convergence Bound of FedGroup without inter-group aggregation]
\label{theo1}
Let Assumption~\ref{assu1} to \ref{assu3} hold and $g,t,E,\bm{w}_t^g,\bm{v}_{t,e}^g$ be defined therein. Then the convergence bound between the federated group model and the virtual group model is $\frac{\delta M}{L}((\eta L+1)^{E}-1)$.
\end{theorem}

Then we extent Theorem~\ref{theo1} to the case where $\eta_g>0$. First we introduce $\tilde{\bm{w}}_t^g$ to represent the model parameter of group $g$ after inter-group aggregation. Then the update of FedGroup with inter-group aggregation can be described as Eq.~(\ref{eq:fedgroup without agg}) and
\begin{equation}
	\tilde{\bm{w}}_t^g = \bm{w}_t^g+\eta_g \sum_{l\in \mathcal{G}, l \neq g}\frac{\bm{w}_t^l}{\| \bm{w}_t^l \|}
\end{equation}

We replace $\bm{w}_t^g$ in Eq.~(\ref{eq:different between group and virtual}) with $\tilde{\bm{w}}_t^g$ and derive

\begin{equation}
\begin{aligned}
	\| \tilde{\bm{w}}_t^g -\bm{v}_{t,e}^g \| &= \| \bm{w}_{t}^{g} - \bm{v}_{t,e}^g + \eta_g \sum_{l\in \mathcal{G}, l \neq g}\frac{\bm{w}_t^l}{\| \bm{w}_t^l\|} \| \\
	&\leq \| \bm{w}_{t}^{g} - \bm{v}_{t,e}^g \| + \eta_g \sum_{l\in \mathcal{G}, l \neq g} \| \frac{\bm{w}_t^l}{\| \bm{w}_t^l\|} \| \\
	&\leq \frac{\delta}{L}((\eta L+1)^{E}-1) + \eta_g (|\mathcal{G}|-1)
\end{aligned}
\end{equation}

Then by the M-Lipschitz continuous of $F_g(\cdot)$ we get the convergence bound of FedGroup with inter-group aggregation:
\begin{equation}
	\label{eq:bound fedgroup with agg}
	\| F_g(\tilde{\bm{w}}_t^g) - F_g(\bm{v}_{t,e}^g) \| \leq \frac{\delta M}{L}((\eta L+1)^{E}-1) + \eta_g (|\mathcal{G}|-1)
\end{equation}

Note that, Eq.~(\ref{eq:bound fedgroup with agg}) degrades to Eq.~(\ref{eq:bound fedgroup without agg}) when $\eta_g=0$ or $|\mathcal{G}|=1$, which means the learning rate of inter-group aggregation is 0 (disabled) or there is only one group in FedGroup (be degraded to FedAvg framework).

